Exploratory Analysis of Federated Learning Methods with Differential Privacy on MIMIC-III

Background: Federated learning methods offer the possibility of training machine learning models on privacy-sensitive data sets, which cannot be easily shared. Multiple regulations pose strict requirements on the storage and usage of healthcare data, leading to data being in silos (i.e. locked-in at healthcare facilities). The application of federated algorithms on these datasets could accelerate disease diagnostic, drug development, as well as improve patient care. Methods: We present an extensive evaluation of the impact of different federation and differential privacy techniques when training models on the open-source MIMIC-III dataset. We analyze a set of parameters influencing a federated model performance, namely data distribution (homogeneous and heterogeneous), communication strategies (communication rounds vs. local training epochs), federation strategies (FedAvg vs. FedProx). Furthermore, we assess and compare two differential privacy (DP) techniques during model training: a stochastic gradient descent-based differential privacy algorithm (DP-SGD), and a sparse vector differential privacy technique (DP-SVT). Results: Our experiments show that extreme data distributions across sites (imbalance either in the number of patients or the positive label ratios between sites) lead to a deterioration of model performance when trained using the FedAvg strategy. This issue is resolved when using FedProx with the use of appropriate hyperparameter tuning. Furthermore, the results show that both differential privacy techniques can reach model performances similar to those of models trained without DP, however at the expense of a large quantifiable privacy leakage. Conclusions: We evaluate empirically the benefits of two federation strategies and propose optimal strategies for the choice of parameters when using differential privacy techniques.

==> sections/ppml.tex <==
\section{Privacy-Preserving Machine Learning Framework}
\label{sec:ppml_appendix}

% Description of the PPML framework
% Packages
% Pipelines
% Interfaces
% DP implementation

\subsection{Differential Privacy}
The DP-SGD, the DP-SVT algorithm is implemented in the ppml Python package and is available out-of-the-box for future models. The implementation also tracks the used privacy budget and can stop the sharing of model weights once a certain threshold has been reached.

\subsubsection{Differential Privacy - Stochastic Gradient Descent}
This method directly introduces differential privacy into the model training by perturbing the model gradients in each backpropagation step. The \textit{opacus} package implements this technique for PyTorch and PyTorch Lightning models, thus we integrated this functionality as a so-called MixIn, which will be available out-of-the-box for any model implemented using the ppml package and PyTorch/PyTroch Lightning. The MixIn class automates the procedure of instantiating a privacy engine and attaching it to the optimizers that track gradients during training. Furthermore, the MixIn class automatically logs the used privacy budget (epsilon) and can stop the model from training once a certain privacy threshold has been reached.

\subsubsection{Differential Privacy - Sparse Vector Technique}
\hl{TODO}



==> styles/latex_templates.tex <==
\begin{comment}
\bgroup
\def\arraystretch{1.5}
\begin{table}[ht]
\begin{center}
    \normalsize
\begin{tabular}{l|l|c|c|c}
\multicolumn{2}{c}{}&\multicolumn{2}{c}{True Interactions}&\\
\cline{3-4}
\multicolumn{2}{c|}{}&Positive&Negative&\multicolumn{1}{c}{}\\
\cline{2-4}
\multirow{2}{*} \phantom{}Predicted & Positive & $TP$ & $FP$ & $\textbf{Precision} = TP / (TP + FP)$\\%[+1pt]
\cline{2-4} Interactions & Negative & $FN$ & $TN$ & \\
\cline{2-4}
%\multicolumn{1}{c}{} \\
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{$\textbf{TPR}, \textbf{Recall} =$} & \multicolumn{1}{c}{$\textbf{FPR} =$} \\ %\multicolumn{1}{c}{$\textbf{F1} = 2TP / (2TP+FP+FN)$}\\
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{$TP / (TP + FN)$} & \multicolumn{1}{c}{$FP / (FP + TN)$}\\
\end{tabular}
    \end{center}
    \caption{Overall baseline demographic and clinical characteristics of all patients with SSc-ILD.\label{table:patient characteristics}}
\end{table}
\egroup
\end{comment}

\begin{table}[htbp]
\begin{center}
    \normalsize
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\textbf{Model}                       & \multicolumn{2}{c|}{\textbf{DS1}} & \multicolumn{2}{c|}{\textbf{DS2}} & \multicolumn{2}{c|}{\textbf{DS3 (CYP)}} & \multicolumn{2}{c}{\textbf{DS3 (NCYP)}} \\ \hline
\textbf{Score}                       & \textbf{AUC}        & \textbf{AUPR}       & \textbf{AUC}        & \textbf{AUPR}       & \textbf{AUC}           & \textbf{AUPR}          & \textbf{AUC}            & \textbf{AUPR}          \\ \hline
\textit{\textbf{AttentionDDI}} (our model)                & \textbf{0.954}      & \textbf{0.924}     & \textbf{0.986}      & \textbf{0.904}      &\textbf{0.989}         & \textbf{0.775}         & \textbf{0.986}          & \textbf{0.890}         \\
\textit{\textbf{NDD}}*                        & 0.954      & 0.922      &\textbf{0.994}    & 0.890       &\textbf{0.994}        &\textbf{0.830}        &\textbf{0.992}         &\textbf{0.947}        \\
\textit{Classifier ensemble}*        & 0.956      &\textbf{0.928}     & 0.936      & 0.487      & 0.990          & 0.541         & 0.986          & 0.756         \\
\textit{Weighted average ensemble}*  & 0.948      & 0.919      & 0.646      & 0.440       & 0.695         & 0.484         & 0.974          & 0.599         \\
\textit{RF}*                         & 0.830       & 0.693      & 0.982      & 0.812      & 0.737         & 0.092         & 0.889          & 0.167         \\
\textit{LR}*                         & 0.941      & 0.905      & 0.911      & 0.251      & 0.977         & 0.487         & 0.916          & 0.472         \\
\textit{Adaptive boosting}*          & 0.722      & 0.587      & 0.904      & 0.185      & 0.830          & 0.143         & 0.709          & 0.150          \\
\textit{LDA}*                        & 0.935      & 0.898      & 0.894      & 0.215      & 0.953         & 0.327         & 0.889          & 0.414         \\
\textit{QDA}*                        & 0.857      & 0.802      & 0.926      & 0.466      & 0.709         & 0.317         & 0.536          & 0.260          \\
\textit{KNN}*                        & 0.730       & 0.134      & 0.927      & 0.785      & 0.590          & 0.064         & 0.603          & 0.235         \\
\textit{\textbf{ISCMF}}\textdagger                     & 0.899      & 0.864      &    -        &      -      & 0.898         & 0.767         & 0.898          & 0.792         \\
\textit{Classifier ensemble}\textdagger       &\textbf{0.957}      & 0.807      &    -        &        -    & 0.990          & 0.541         & 0.986          & 0.756         \\
\textit{Weighted average ensemble}\textdagger & 0.951      & 0.795      &     -       &      -      & 0.695         & 0.484         & 0.974          & 0.599         \\
\textit{Matrix perturbation}\textdagger       & 0.948      & 0.782      &    -        &      -      &        -       &       -        &          -      &        -       \\
\textit{Neighbor Recommender}\textdagger      &          -  &    -        &      -      &    -        & 0.953         & 0.126         & 0.904          & 0.295         \\
\textit{Label Propagation}\textdagger         &    -        &        -    &      -      &    -        & 0.952         & 0.126         &          -      &        -       \\
\textit{Random walk}\textdagger               &      -      &    -        &      -      &    -        &      -         &         -      & 0.895          & 0.181        
\end{tabular}
    \end{center}
    \caption[]
    {\tabular[t]{@{}l@{}}Model evaluation scores for all datasets.\\
    *: scores from \cite{rohani_drug-drug_2019}, \textdagger: scores from \cite{rohani_iscmf_2020}\endtabular
    \label{table:model_scores_DS_all}}
\end{table}

==> supplements/List_of_figures.tex <==


M3: could be seed specific
1. ho_epoch_vs_round -  
2. ho_centralized
3. he_epoch_vs_round
4. he_centralized
5. he_fedprox (all combination of epoch_vs_round)
6b.ho_dp_sgd
6a.ho_dp_sgd (Run further experiments which did not converge)
7. ho_dp_svt


CLL: (could be seed specific)
D: 1. ho_epoch_vs_round
M: 2. ho_centralized
D: 3. he_epoch_vs_round
M: 4. he_centralized
5. he_fedprox (all combination of epoch_vs_round)
6b.ho_dp_sgd
6a.ho_dp_sgd (Run further experiments which did not converge)
7. ho_dp_svt


CLL splits:
Homogeneous:
 Final_ratio: 0.9990118577075099
site1_ho_50: 0.19485657764589515
site2_ho_50: 0.1956521739130435
 Final_ratio: 0.6663920922570017
site1_ho_40: 0.19530284301606923
site2_ho_60: 0.19522240527182866
 Final_ratio: 0.42766407904022585
site1_ho_30: 0.19471947194719472
site2_ho_70: 0.19548341566690192
 Final_ratio: 0.24953675108091414
site1_ho_20: 0.19554455445544555
site2_ho_80: 0.19518221124150711
 Final_ratio: 0.11092806150466776
site1_ho_10: 0.19306930693069307
site2_ho_90: 0.19549697968149368
 Final_ratio: 0.05254942767950052
site1_ho_05: 0.19801980198019803
site2_ho_95: 0.19510926118626432

Heterogeneous splot:
 Final_ratio: 0.6666666666666666, sizes: s1: 1011, s2: 1012
site1_he_40: 0.1562809099901088
site2_he_60: 0.2341897233201581
 Final_ratio: 0.4311594202898551, sizes: s1: 1011, s2: 1012
site1_he_30: 0.11770524233432245
site2_he_70: 0.2727272727272727
 Final_ratio: 0.25, sizes: s1: 1011, s2: 1012
site1_he_20: 0.0781404549950544
site2_he_80: 0.31225296442687744
 Final_ratio: 0.11267605633802817, sizes: s1: 1011, s2: 1012
site1_he_10: 0.03956478733926805
site2_he_90: 0.35079051383399207
 Final_ratio: 0.05333333333333334, sizes: s1: 1011, s2: 1012
site1_he_05: 0.019782393669634024
site2_he_95: 0.3705533596837945

==> tables/test.tex <==
% Homogeneous data distribution table
\centering
\begin{tabular}{*8c}
    \toprule
    \multicolumn{2}{c}{\textbf{Icon}} & 
    \includegraphics[width=0.07\textwidth]{figures/icons/ho_0.png} &
    \includegraphics[width=0.07\textwidth]{figures/icons/ho_1.png} &
    \includegraphics[width=0.07\textwidth]{figures/icons/ho_2.png} &
    \includegraphics[width=0.07\textwidth]{figures/icons/ho_3.png} &
    \includegraphics[width=0.07\textwidth]{figures/icons/ho_4.png} &
    \includegraphics[width=0.07\textwidth]{figures/icons/ho_5.png} \\
    \toprule
    
    \multirow{2}{*}{\makecell{Samples \\ ratio (\%)}} & \textbf{Site \#1} & 50 & 40 & 30 & 20 & 10 & 5 \\
    \midrule
     & \textbf{Site \#2} & 50 & 60 & 70 & 80 & 90 & 95 \\
     \bottomrule
\end{tabular}
\vspace{1ex}

